Observer Design for an Inertia Wheel Pendulum with Static Friction

A state observer design for the inertia wheel pendulum considering static friction of the actuated inertia disc is presented. The frictional force is modeled by the Stribeck effect, with two separate differential equations describing the sticking and non-sticking system, respectively. The transition between the two scenarios is in general determined by a static friction condition. Three proposed observers are designed for both the sticking and non-sticking model. Depending on the probability of the respective model given a current measurement, the more likely is selected for state estimation. The performance is demonstrated on a laboratory demonstrator, where the observers including the proposed probabilistic model selection are compared.

==> figures/plot_observer_overview2.tex <==
 %!TEX root = ifacconf_mathmod2022_B.tex

\tikzsetnextfilename{\currfilebase}
\begin{tikzpicture}
%	\hspace*{-0.2cm}
	
	\begin{axis}[
	name = ov1,
	width=8.4cm,
	height=3.5cm,
	ylabel={$\varphi_{1}$ / \SI{}{\radian}},
	xmin=0, xmax=30,
	ymin=-6.81, ymax=0,
	xtick={0,5,10,15,20,25,30},
	ytick = {-2*pi,-1.5*pi,-pi,-0.5*pi,0},
	yticklabels = {$- 2\pi$, $-\frac{3}{2}\pi$,$- \pi$,$\frac{ 1}{2}\pi$, $ 0$},
	legend pos=north west,
	ymajorgrids=true,
	xmajorgrids=true,
	grid style=dashed,
	anchor=above north
	]
	
	

	
	
	\addplot+[color=red,	mark=none, line width=0.4mm, each nth point=\nthpoint] table[x=time, y=data (phi1), col sep=comma] {data_meas.csv}; 
	
	\addplot+[color=green!60!black,dashed, mark=none, line width=0.4mm, each nth point=\nthpoint] table[x=time, y expr ={ \thisrow{data (phi1)}}, col sep=semicolon] {data_NLOWPED_observer.csv};
	
	\addplot+[color=orange,dashed, mark=none, line width=0.4mm, each nth point=\nthpoint] table[x=time, y expr ={ \thisrow{data (phi1)}}, col sep=semicolon] {data_EKF_observer.csv};
	
	\addplot+[color=cyan,dotted, mark=none, line width=0.4mm, each nth point=\nthpoint] table[x=time, y expr ={ \thisrow{data (phi1)}}, col sep=semicolon] {data_LIN_observer.csv}; \label{ps3}
	
	
	\end{axis}
	
	
	
	\begin{axis}[
	name = p1,
	thick,
	%no markers,
	width=8.4cm,
	height=4cm,
	ylabel={$\omega_{2}$ / \SI{}{\radian \per \second}},
	xmin=0, xmax=30,
	ymin=-3, ymax=3,
	xtick={0,5,10,15,20,25,30},
	ytick={-3, -2,-1,0,1,2.0,3},
	xmin=0, xmax=30,
	ymin=-4, ymax=4,
	xtick={0,5,10,15,20,25,30},
	ytick={-4, -2,0,2,4},	
	legend pos=north east,
	ymajorgrids=true,
	xmajorgrids=true,
	grid style=dashed,
	at=(ov1.below south),
	axis on top=true,
	anchor=above north
	]
	
	\addplot+[color=red,mark=none, line width=0.4mm] table[x=time, y=data (omega2), col sep=comma, each nth point=\nthpoint] {data_meas.csv}; \label{ss}
	
	%	\addlegendentry{EKF};
	
	%	\addplot+[color=orange,mark=none, line width=0.4mm] table[x=time, y=data (omega2), col sep=semicolon, each nth point=\nthpoint] {data_EKF_observer.csv};
	
	%	\addplot+[name path = A,color=red,line width = 0.00001mm] table[x = time, y expr ={ \thisrow{state}==1?4:-4}, col sep=semicolon]{data_EKF_observer.csv};
	
	%	\addplot+[name path = B,color=green,line width = 0.00001mm] table[x = time, y expr ={ \thisrow{state}==1?-4:4}, col sep=semicolon]{data_EKF_observer.csv};
	
	%	\addplot[name path = G,mark=none, line width = 0.00001mm] coordinates {(0,-4) (30,-4)};
	
	%	\addplot+[red!10] fill between[of=A and G];
	%	\addplot+[green!10] fill between[of=B and G];
	\end{axis}


\end{tikzpicture}

